Camera-Space Hand Mesh Recovery via Semantic Aggregation and Adaptive 2D-1D Registration

Recent years have witnessed significant progress in 3D hand mesh recovery. Nevertheless, because of the intrinsic 2D-to-3D ambiguity, recovering camera-space 3D information from a single RGB image remains challenging. To tackle this problem, we divide camera-space mesh recovery into two sub-tasks, i.e., root-relative mesh recovery and root recovery. First, joint landmarks and silhouette are extracted from a single input image to provide 2D cues for the 3D tasks. In the root-relative mesh recovery task, we exploit semantic relations among joints to generate a 3D mesh from the extracted 2D cues. Such generated 3D mesh coordinates are expressed relative to a root position, i.e., wrist of the hand. In the root recovery task, the root position is registered to the camera space by aligning the generated 3D mesh back to 2D cues, thereby completing cameraspace 3D mesh recovery. Our pipeline is novel in that (1) it explicitly makes use of known semantic relations among joints and (2) it exploits 1D projections of the silhouette and mesh to achieve robust registration. Extensive experiments on popular datasets such as FreiHAND, RHD, and Human3.6M demonstrate that our approach achieves stateof-the-art performance on both root-relative mesh recovery and root recovery. Our code is publicly available at https://github.com/SeanChenxy/HandMesh.

==> Tables/tab10.tex <==
\begin{table}[!t]
\small
\renewcommand{\arraystretch}{1.}
\setlength\tabcolsep{8pt}
\centering
\begin{tabular}{c  c c c c }
\hline
Method             & J $\downarrow$ & PJ $\downarrow$ & V $\downarrow$ & PV $\downarrow$ \\
\hline
\multicolumn{4}{l}{\emph{trained with Human3.6M}}\\
CMR-PG (ResNet18)  & 67.9  & 49.9  & 80.5 & 62.8 \\
CMR-PG (ResNet50)  & 69.8  & 47.9  & 83.9 & 61.9  \\
\hline
\multicolumn{4}{l}{\emph{trained with Human3.6M+COCO}}\\
CMR-P (ResNet18, w/ \emph{hp})  & 62.5  & 46.8  & 72.8 & 58.3  \\
CMR-P (ResNet18, w/ \emph{group(hp)})  & 61.1  & 45.3  & 71.9 & 56.8  \\
CMR-PG (ResNet18)  & 59.0  & 44.7  & 70.8 & 56.4  \\
CMR-PG (ResNet50)  & 57.3  & 42.6  & 68.7 & 54.1  \\
\hline
\end{tabular}
\caption{Results of root-relative mesh recovery on Human3.6M. ``J, PJ, V, PV'' denote MPJPE, PA-MPJPE, MPVPE, PA-MPVPE.}
\label{tab:h36m_full}
\vspace{-0.2cm}
\end{table}

==> Tables/tab11.tex <==
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.}
\small
%\setlength\tabcolsep{3.2pt}
\centering
\begin{tabular}{c  c | c c c c c c}
\hline
Method       & Backbone   & PA-MPJPE $\downarrow$ &J-AUC $\uparrow$ & PA-MPVPE $\downarrow$ & V-AUC $\uparrow$ & F@5 mm $\uparrow$ & F@15 mm $\uparrow$ \\
\hline
Boukhayma \etal (CVPR2019) \cite{bib:Boukhayma19} & ResNet50 & 35.0 & 0.351 & 13.2 & 0.738 & 0.427 & 0.895 \\
ObMan (CVPR2019) \cite{hasson2019learning}	                 & ResNet18	& 13.3 & 0.737 & 13.3 & 0.736 & 0.429 & 0.907 \\
MANO CNN (ICCV2019) \cite{bib:FreiHand}	         & ResNet50 & 11.0 & 0.783 & 10.9 & 0.783 & 0.516 & 0.934 \\
YotubeHand (CVPR2020) \cite{bib:YoutubeHand}	     & ResNet50	& 8.4  & 0.834 & 8.6  & 0.830 & 0.614 & 0.966 \\
Pose2Mesh (ECCV2020) \cite{bib:Pose2Mesh}          & $-$      & 7.7  & 0.852 & 7.8  & 0.850 & 0.674 & 0.969 \\
I2L-MeshNet (ECCV2020) \cite{bib:I2L}              & ResNet50 & 7.4  & 0.854 & 7.6  & 0.850 & 0.681 & 0.973 \\
%2nd in benchmark         & -        & 7.3  & 0.854 & -    & -     & -     & - \\
\hline
CMR-SG	           & ResNet18	& 7.5  & 0.851 & 7.6  & 0.850 & 0.685 & 0.971 \\
CMR-PG             & ResNet18 & 7.4  & 0.853 & 7.5  & 0.851 & 0.687 & 0.973 \\
CMR-SG             & ResNet50 & 7.0  & 0.860 & 7.1  & 0.858 & 0.706 & 0.976 \\
CMR-PG             & ResNet50 & \bf 6.9  & \bf 0.863 & \bf 7.0  & \bf 0.861 & \bf 0.715 & \bf 0.977 \\
\hline
\end{tabular}
\caption{Results of root-relative mesh recovery on FreiHAND. ``J-AUC, V-AUC'' denote AUC of 3D joint and mesh vertex, respectively. ``F@5 mm, F@15 mm'' is the harmonic mean between recall and precision between two meshes \emph{w.r.t.} a specific distance threshold.}
\label{tab:freihand_align}
%\vspace{-0.2cm}
\end{table*}


==> Tables/tab12.tex <==
\begin{table*}[!t]
\small
\renewcommand{\arraystretch}{1.}
%\setlength\tabcolsep{4.2pt}
\centering
\begin{tabular}{c  c | c c c c c c}
\hline
Method       & Backbone   & CS-MPJPE $\downarrow$ &J-AUC $\uparrow$ & CS-MPVPE $\downarrow$ & V-AUC $\uparrow$ & F@5 mm $\uparrow$ & F@15 mm $\uparrow$ \\
\hline
ObMan (CVPR2019) \cite{hasson2019learning} & ResNet18   & 85.2 & 0.168 & 85.4 & 0.167 & 0.087 & 0.305 \\
ManoCNN (ICCV2019) \cite{bib:FreiHand}          & ResNet50	& 71.3 & 0.185 & 71.5 & 0.184 & 0.102 & 0.345 \\
I2L-MeshNet (ECCV2020) \cite{bib:I2L}      & ResNet50	& 60.3 & 0.233 & 60.4 & 0.232 & 0.132 & 0.394 \\
\hline
CMR-PG             & ResNet18 & 50.6 & 0.290 & 50.6 & 0.289 & 0.155 & 0.474 \\
CMR-SG             & ResNet18 & 49.7 & 0.295 & 49.8 & 0.294 & 0.159 & 0.481 \\
CMR-PG             & ResNet50 & 48.9 & 0.304 & 49.0 & 0.303 & 0.163 & 0.488 \\
CMR-SG             & ResNet50 & \bf 48.8 & \bf0.307 & \bf48.9 & \bf0.306 & \bf0.166 & \bf0.492 \\
\hline
\end{tabular}
\caption{Results of camera-space mesh recovery on FreiHAND. Please refer to Table~\ref{tab:freihand_align} for metrics explanation.}
\label{tab:freihand_abs}
%\vspace{-0.3cm}
\end{table*}


==> Tables/tab7.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.}
\setlength\tabcolsep{4.2pt}
\centering
\begin{tabular}{c  c | c c c c c c}
\hline
Method       & Backbone   & PA-MPJPE $\downarrow$ &J-AUC $\uparrow$ & PA-MPVPE $\downarrow$ & V-AUC $\uparrow$ & F@5 mm $\uparrow$ & F@15 mm $\uparrow$ \\
\hline
Boukhayma et al. (CVPR2019) \cite{bib:Boukhayma19} & ResNet50 & 35.0 & 0.351 & 13.2 & 0.738 & 0.427 & 0.895 \\
ObMan (CVPR2019) \cite{bib:ObMan}	                 & ResNet18	& 13.3 & 0.737 & 13.3 & 0.736 & 0.429 & 0.907 \\
MANO CNN (ICCV2019) \cite{bib:FreiHand}	         & ResNet50 & 11.0 & 0.783 & 10.9 & 0.783 & 0.516 & 0.934 \\
YotubeHand (CVPR2020) \cite{bib:YoutubeHand}	     & ResNet50	& 8.4  & 0.834 & 8.6  & 0.830 & 0.614 & 0.966 \\
Pose2Mesh (ECCV2020) \cite{bib:Pose2Mesh}          & $-$      & 7.7  & 0.852 & 7.8  & 0.850 & 0.674 & 0.969 \\
I2L-MeshNet (ECCV2020) \cite{bib:I2L}              & ResNet50 & 7.4  & 0.854 & 7.6  & 0.850 & 0.681 & 0.973 \\
%2nd in benchmark         & -        & 7.3  & 0.854 & -    & -     & -     & - \\
\hline
CMR-SG	           & ResNet18	& 7.5  & 0.851 & 7.6  & 0.850 & 0.685 & 0.971 \\
CMR-PG             & ResNet18 & 7.4  & 0.853 & 7.5  & 0.851 & 0.687 & 0.973 \\
CMR-SG             & ResNet50 & 7.0  & 0.860 & 7.1  & 0.858 & 0.706 & 0.976 \\
CMR-PG             & ResNet50 & \bf 6.9  & \bf 0.863 & \bf 7.0  & \bf 0.861 & \bf 0.715 & \bf 0.977 \\
\hline
\end{tabular}
\caption{Results of root-relative mesh recovery on FreiHAND. ``J-AUC, V-AUC'' denote AUC of 3D joint and mesh vertex, respectively. ``F@5 mm, F@15 mm'' indicate the percentage of correct mesh vertexes that fall within a specific error threshold.}
\label{tab:freihand_align}
\end{table*}

==> Tables/tab8.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.}
\setlength\tabcolsep{5.2pt}
\centering
\begin{tabular}{c  c | c c c c c c}
\hline
Method       & Backbone   & CS-MPJPE $\downarrow$ &J-AUC $\uparrow$ & CS-MPVPE $\downarrow$ & V-AUC $\uparrow$ & F@5 mm $\uparrow$ & F@15 mm $\uparrow$ \\
\hline
ObMan (CVPR2019) \cite{bib:ObMan}	     & ResNet18 & 85.2 & 0.168 & 85.4 & 0.167 & 0.087 & 0.305 \\
I2L-MeshNet (ECCV2020) \cite{bib:I2L} & ResNet50	& 60.3 & 0.233 & 60.4 & 0.232 & 0.132 & 0.394 \\
\hline
CMR-PG             & ResNet18 & 50.6 & 0.290 & 50.6 & 0.289 & 0.155 & 0.474 \\
CMR-SG             & ResNet18 & 49.7 & 0.295 & 49.8 & 0.294 & 0.159 & 0.481 \\
CMR-PG             & ResNet50 & 48.9 & 0.304 & 49.0 & 0.303 & 0.163 & 0.488 \\
CMR-SG             & ResNet50 & \bf 48.8 & \bf0.307 & \bf48.9 & \bf0.306 & \bf0.166 & \bf0.492 \\
\hline
\end{tabular}
\caption{Results of camera-space mesh recovery on FreiHAND. Referring to Table~\ref{tab:freihand_align} for metrics explaination.}
\label{tab:freihand_abs}
\end{table*}

